Identifying Helpful Sentences in Product Reviews

In recent years online shopping has gained momentum and became an important venue for customers wishing to save time and simplify their shopping process. A key advantage of shopping online is the ability to read what other customers are saying about products of interest. In this work, we aim to maintain this advantage in situations where extreme brevity is needed, for example, when shopping by voice. We suggest a novel task of extracting a single representative helpful sentence from a set of reviews for a given product. The selected sentence should meet two conditions: first, it should be helpful for a purchase decision and second, the opinion it expresses should be supported by multiple reviewers. This task is closely related to the task of Multi Document Summarization in the product reviews domain but differs in its objective and its level of conciseness. We collect a dataset in English of sentence helpfulness scores via crowd-sourcing and demonstrate its reliability despite the inherent subjectivity involved. Next, we describe a complete model that extracts representative helpful sentences with positive and negative sentiment towards the product and demonstrate that it outperforms several baselines.

==> data.tex <==
% \rl{I think this part repeats the introduction and should be either removed or incorporated into the intro}
% As mentioned in the introduction, customers rely on other customers reviews before taking purchase decisions. 
% Customers reviews are good source of information and sentiment about a product and, by using them, individuals gain more confidence toward purchasing a particular product --- when sentiment is positive, and the additional information contained in the reviews aligns with the customer's needs --- or, encourage them to search for an alternative product --- if sentiment is negative or the additional information conflicts with their needs.
% \rl{end comment}

We consider a subset of 123 products from the Amazon Customer Reviews Dataset~\cite{reviews}.
The products were arbitrarily selected, so each of them has at least 100 customer reviews and they (approximately) equally represent 6 different categories (Toys, Books, Movies, Music, Camera and Electronics).
We split the reviews into sentences and randomly selected a train set containing 20,000 sentences, and a test set containing 3,000 sentences.
We asked annotators to vote whether each sentence is helpful for the purposes of purchasing decision. 
The options we provided for the annotators are \textbf{Not Helpful} (0), \textbf{Somewhat Helpful} (1), or \textbf{Very Helpful} (2). 
As the final helpfulness score of each sentence we take the average scoring given by the annotators.
Figure~\ref{fig:annotation} displays a single annotation task as presented to the annotators.
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{annotation.png}
    \caption{A single annotation as presented to the annotators.\label{fig:annotation}}
\end{figure}
We used 10 different annotators to annotate each example from our training set and 30 different annotators to annotate each example from our test set.
Table~\ref{tab:top-bottom-sentences} presents the 5 most helpful and the 5 least helpful sentences
from our test set as perceived by the annotators and Figure~\ref{fig:help-dist} depicts the helpfulness distribution among our train and test sets.

\begin{table}[ht]
    \centering
    \begin{tabular}{@{}p{0.78\linewidth}r@{}} \toprule
    Sentence & Helpfulness \\
    \midrule
% 
    Really great headphones, especially for \$25, but honestly, they sound better than my gaming headset and my DJ headphones in many respects. & 1.97 \\
    \midrule
    Good sound quality, stays in my ears with vigorous activity. & 1.93 \\
    \midrule
    Simple to install and a great sound, i put these under the eaves of my garage and connected them into an old stereo I had. & 1.9 \\
    \midrule
    This is an amazing book which I will read and reread to really absorb what it has to offer; What I like the most are the self exercises; The author doesn't just suggest what to do to change your self image and achieve success, but how to do it with practice exercises. & 1.9 \\
    \midrule
    I love the sound quality and the shoelace cord, which is easy to keep untangled. & 1.9 \\
    \midrule
% 
    I know not everyone read the book. & 0.05 \\
    \midrule
    I rarely write Amazon reviews & 0.03 \\
    \midrule
    jacket on, jacket off, etc & 0.03 \\
    \midrule
    Here's my take on this flash unit: & 0.03 \\
    \midrule
    Any thoughts from others? & 0 \\
    \bottomrule        
    \end{tabular}
    \caption{The 5 most helpful and 5 most unhelpful sentences from our test set as perceived by annotators\label{tab:top-bottom-sentences}}
\end{table}

\begin{figure}[ht]
    \begin{tikzpicture}
        \begin{axis}[
            width=1\linewidth,
            height=7.5cm,
            legend style={at={(0.5,1)},anchor=south,draw=none},
            legend entries={Train,Test,Random},
            legend columns={3},
            grid style=dashed,            
            no markers,
            very thick,
            xlabel=Helpfulness,
            ymajorgrids=true,
            ylabel=Frequency,
        ]
            \addplot[orange,smooth, thick] table [] {data/train_hist.csv};
            \addplot[cyan, dashed, smooth, thick] table [] {data/test_hist.csv};
            \addplot[green, dotted, smooth, thick] table [] {data/random_hist.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{\label{fig:help-dist}
        Helpfulness distribution among the train and test sets.
        The green, dotted line represent the expected distribution if the annotators would have chosen an answer uniformly at random.
    }
\end{figure}

\rl{alternative description for reliability analysis}
As mentioned earlier, rating sentence helpfulness is a highly subjective task which means one cannot expect honest raters to agree most of the time. Nevertheless, we argue that the data we collected is reliable and demonstrate it through three separate experiments. First, we compute a standard inter-annotator agreement measure based on Pearson correlation and observe a moderate agreement. Next, we show that the data is internally consistent by measuring the score variance within sets of semantically similar sentences and showing that it is significantly lower than the score variance of the general population. Finally, we show that our scores agree with the opinions of real customers by contrasting them with review helpfulness votes.

\textbf{Inter Annotator Agreement} was computed in the spirit of the analysis performed in \cite{snow2008}. For each annotator, we restrict the data to the set of rows that he/she completed and compute the Pearson correlation between his/her answers against the average of all other annotators. Finally, we take the average across all after removing the worst $10\%$ annotators according to the method of \cite{DawidAndSkene}. The average Pearson correlation on the train set (10 annotators per row) is $0.44\pm0.01$ and on the test set (30 annotators per row) it is $0.57\pm0.02$. These moderate scores are not surprising given the subjective nature of this task and are comparable, for example, with the scores reported in \cite{snow2008} for the highly subjective Affective Text Analysis task.
We also randomly split the annotators into two disjoint sets and calculated the correlation
between the corresponding scores.
There was a correlation of $0.49$ for the train set (5 annotators in each group) and $0.81$ for the 
test set (15 annotators in each group). We elaborate on our choice to use $10/30$ ratings per row in the train/test sets respectively in Section~\ref{sec:eval}.

\textbf{Internal Consistency}

\textbf{Sentence Helpfulness vs. Review Helpfulness}

\rl{end intro}

Next we describe the steps we made to verify that our helpfulness annotations capture a real signal.
To begin, we randomly split the annotators into two disjoint groups and calculated the correlation
between the corresponding scores.
There was a correlation of 0.49 for the train set (5 annotators in each group) and 0.81 for the 
test set (15 annotators in each group). 
We elaborate on the effect of the number of annotators per sentence in Section~\ref{sec:eval}.
In contrast, when simulating 30 annotators that vote by choosing an answer uniformly at random the expected correlation is 0 and the helpfulness distribution is more concentrated as can be seen in Figure~\ref{fig:help-dist}

To further validate that the annotators separate the helpful sentences from the unhelpful ones we 
compared the helpful score obtained from the annotators with review helpfulness votes taken from Amazon
website. 
We split the reviews into two sets, helpful and unhelpful, where in the helpful set we considered all the
reviews with at least 50 helpful votes and in the negative set we considered all the reviews with no 
helpful votes. 
We then took random selection of 500 sentence from each set and calculated the mean helpful score, the ratio of sentences in each set with helpful score greater than 1, 1.5, 1.75 respectively.
Table~\ref{tab:contrast-data} describe the data and Table~\ref{tab:contrast-result} describe the results
of the experiment.

\begin{table}[ht]   
\centering
\begin{tabular}{@{}lcccc@{}} \toprule
    & \# Helpful & \# Reviews & \# Sentences & Mean \\
    & Votes & & & Sentences\\
    \cmidrule{2-5}
    Helpful Set     & 0         & 3803  & 22030 & 5.79    \\
    Unhelpful Set   & $\ge$ 50  & 101   & 5032  & 49.82   \\
    \bottomrule
\end{tabular}
    \caption{
        Contrasting Sentence Helpfulness Score with Review Helpfulness votes --- Dataset%
        \label{tab:contrast-data}
    }
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{@{}lccc@{}} \toprule
    & Mean & Ratio & Ratio \\
    & Score & Score $>1$ & Score $>1.5$\\
    \cmidrule{2-4}
    Helpful Set     & 1.21  & 70\%  & 18\% \\
    Unhelpful Set   & 1.15  & 64\%  & 14\% \\
    \bottomrule
\end{tabular}
    \caption{
        Contrasting Sentence Helpfulness Score with Review Helpfulness votes --- Results%
        \label{tab:contrast-result}}
\end{table}

The difference in the mean helpfulness score is statistical significant with a p-value of approximately 0.0079 (t-test with an equal variance assumption as well as t-test with different variance assumption, a.k.a Welch’s t-test)

The statistical significant difference between the helpfulness sco\-res of the two sets shows that there exists a relation between our notion of sentence helpfulness and the customer perceived review helpfulness.
However, the relation is not very strong. We observe that helpful reviews may contain unhelpful sentences and vice versa.
The average length (in sentences) of a helpful review is almost 10 times longer than a non helpful review. We conjecture that the two notions of helpfulness differ:  a helpful sentence is a micro summary of a helpful review while a helpful review is one that includes details and justifies its summary.
Finally, to rule out the possibility that annotators confused ``helpfulness'' with the sentiment of the sentence or its length we compared the correlations between them.
The correlation between the length of the sentence and its helpfulness score given by the annotators is 0.29.
For the sentiment we measured the correlation separately for the positive sentences and the negative ones. 
The correlation for the positive sentences between its positively score and its helpfulness score is 0.34.
The correlation for the negative sentences between its negatively score and its helpfulness score is 0.31.
The above show that sentiment and length characterize helpful sentences to some degree, but clearly neither of them can be considered as a synonym to helpfulness.

==> report.tex <==
\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000W7F5SS.jpg}}
& \textbf{That said, the actual movie is wonderful and a joy to watch!} & 1.52\\
\cmidrule{2-3}
& That in and of itself is enough to make me love this movie. & 0.92 \\
& The movies have all been most enjoyable and worthwhile. & 0.89 \\
& Its a great movie and has great action in it! & 0.89 \\
& Great Movie, glad to finally have it in my collection. & 0.88 \\
& I was really impressed with the acting in this movie. & 0.88 \\
& Great movie, if you're a HP movie fan you're sure to enjoy. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0451232852.jpg}}
& \textbf{I love these books and find them well-researched with some great characters.} & 1.55\\
\cmidrule{2-3}
& I really enjoy reading great books like Follett's that are historically accurate and filled with colorful characters who you grow to love or sometimes even grow to dispise. & 0.93 \\
& The writing is very good, and the well-researched history is very interesting. & 0.9 \\
& I enjoy historical fiction when well researched and that he does very well. & 0.9 \\
& I thoroughly enjoyed this book. & 0.89 \\
& He loves this author and this series. & 0.89 \\
& I enjoyed this book very much. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00LOY6G1I.jpg}}
& \textbf{This is a really fun toy, you really can handle and play with the bubbles!} & 1.61\\
\cmidrule{2-3}
& Very easy to make the bubbles and had fun with them! & 0.9 \\
& The kids loved the Juggle Bubble. & 0.88 \\
& This is one of the most fun bubble toys EVER!!! & 0.87 \\
& Item delivered quickly and children love playing with the bubbles. & 0.87 \\
& My family enjoyed playing with these bubbles very much! & 0.87 \\
& The Juggle-Bubble, I am happy to announce works and also fun for the kids. & 0.86 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00002E220.jpg}}
& \textbf{This is simply a terrific movie that has it all, a wonderful cast, an intriguing story line, beautiful scenery, and an enjoyable soundtrack.} & 1.59\\
\cmidrule{2-3}
& The direction and soundtrack complement the acting, direction and setting to form a movie that is splendidly well-done across the board. & 0.93 \\
& The friendships formed,the evolving romance, the cinematogrpahy, the musical score, and the heartwarming story all combined for a wonderful film. & 0.92 \\
& The acting is great, the scenery is fantastic and the music is at the top. & 0.9 \\
& This is a fantastic movie .. story, scenery, and music and well acted by Tom Berenger (as always) and Barbara Hershey. & 0.89 \\
& Direction and the sound track support and complement the acting and scenery, making the movie a wonderful experience. & 0.89 \\
& I believe the acting is top-notch, the settings are magnificent, the music touches me deeply. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000002GJH.jpg}}
& \textbf{This is one of the best CDs i ever heard, and that's an understatement.} & 1.53\\
\cmidrule{2-3}
& This is, perhaps, the best CD I've ever heard. & 0.95 \\
& Say Hello 2 Heaven; undoubtedly, this is the best song on the album. & 0.9 \\
& One Of The Greatest CD's Ever! & 0.9 \\
& this is the greatest single album i have ever heard. & 0.89 \\
& This album is Mind Blowing, You have the best of both worlds here. & 0.88 \\
& His voice is the most powerful around, and in my opinion, this album has his best work on it. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00081NX5U.jpg}}
& \textbf{I think they sound great, a very well balanced sound and volume to spare.} & 1.63\\
\cmidrule{2-3}
& The speakers sound great and look good too. & 0.93 \\
& The sound quality is really good and the value is excellent. & 0.92 \\
& The sound quality is very good. & 0.92 \\
& They really do deliver good sound. & 0.92 \\
& They have decent sound output. & 0.92 \\
& They sound great and look nice as well. & 0.92 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B003G9ZQQA.jpg}}
& \textbf{This set is very well made and is a pleasure to use.} & 1.59\\
\cmidrule{2-3}
& Am very pleased with the product. & 0.92 \\
& We have enjoyed this set very much. & 0.92 \\
& Liked this version as it is well done and good quality. & 0.91 \\
& This is a really fun game and this version is well built. & 0.91 \\
& Was very pleased with this set. & 0.91 \\
& I am very happy with this set. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0007U00XK.jpg}}
& \textbf{The picture quality is excellent, and the handling is great.} & 1.67\\
\cmidrule{2-3}
& Color and contrast is very good. & 0.92 \\
& I am pleased overall with this lens. & 0.91 \\
& The lens is very well constructed and the saturation that the lens adds to the photos is very welcoming. & 0.91 \\
& The photos are nice and sharp, the focus works as well as it needs to and the photos come out great. & 0.9 \\
& Wonderful lens, getting great shots with it! & 0.9 \\
& Very, very satisfied with the quality of the images - the sharpness is excellent. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B002ZG99CC.jpg}}
& \textbf{This was a fantastic film and it was very well done and very entertaining.} & 1.59\\
\cmidrule{2-3}
& I found this movie to be fun and enjoyable. & 0.9 \\
& Like the original, I found this to be an enjoyable, uplifting film. & 0.9 \\
& Overall this  movie was GREAT. & 0.9 \\
& Without a doubt, this is a magnificent movie, worth seeing. & 0.89 \\
& The movie was excellently done!!! & 0.89 \\
& I totally agree that this movie was fun, exciting, and beautiful to watch - definitely worth the money. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0061208493.jpg}}
& \textbf{Well pleased with this book and great service.} & 1.55\\
\cmidrule{2-3}
& The book is pleasingly produced, and the content, of course, is excellent. & 0.94 \\
& I very much enjoy this book so far! & 0.93 \\
& Wonderful and definitely worth the read. & 0.9 \\
& Awesome book, awesome quality. & 0.89 \\
& I am VERY pleased with my purchase. & 0.88 \\
& Also I love the pages of this book. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0470474874.jpg}}
& \textbf{This is an excellent, easy to follow manual.} & 1.62\\
\cmidrule{2-3}
& this authore is very easy to understand . & 0.95 \\
& Very comprehensive and easy to use. & 0.94 \\
& It is very well written and easy to follow. & 0.94 \\
& Subject is very detailed and easy to follow. & 0.94 \\
& It is well written and easy to understand. & 0.94 \\
& This book is excellent and explains everything in an easy-to-understand format. & 0.94 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0000DZTIW.jpg}}
& \textbf{The movie theme was strengthened by the artful use of this soundtrack, and it is a pleasure to listen to.} & 1.52\\
\cmidrule{2-3}
& I loved both the movie and the soundtrack. & 0.91 \\
& I loved the movie , and also the music....If you loved the music in the movie you will love this soundtrack...I  Recommend this.. & 0.9 \\
& I LOVED THE MOVIE, I LOVE THE SOUND TRACK…. & 0.9 \\
& i enjoyed the movie, and i really enyou the music. & 0.89 \\
& The music in this really suits the picture well and aids in transporting viewers to another world. & 0.88 \\
& I love the way the music mirrors the film. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00004UFOO.jpg}}
& \textbf{I love the multitude of colors and they are such good quality.} & 1.62\\
\cmidrule{2-3}
& Love the variety and vibrancy of these colors. & 0.95 \\
& And they love the wide assortment of colors. & 0.94 \\
& I love the selection of colors. & 0.94 \\
& THEY BLEND BEAUTIFULLY AND THE COLORS ARE VIBRANT. & 0.92 \\
& I am very impressed with the amount of markers and variety of colors available. & 0.92 \\
& Plenty of colors to choose from and they work great. & 0.92 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0006ZOV5E.jpg}}
& \textbf{This Album is Great...Melodies are So Soothing and Insanely Beautiful!} & 1.58\\
\cmidrule{2-3}
& These songs are heartfelt, genuine, honest, beautiful, magical...in a word, marvelous. & 0.92 \\
& Eisley's unique sound is so soothing, refreshing, and at the same time slightly rockin. & 0.89 \\
& Their voices combine to create such a euphoric, ethereal blend, it's beautiful. & 0.89 \\
& Eisley's unique melodies, emotional and beautiful voices, unusual and sincere lyrics and interweaving harmonies will win your soul. & 0.88 \\
& The lyrics are so cute and inspirational. & 0.87 \\
& Eisley's sound is ethereal, wistful, and refreshing. & 0.86 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000NP46K2.jpg}}
& \textbf{The quality of this lens is just incredible.} & 1.64\\
\cmidrule{2-3}
& The picture quality is simply amazing! & 0.94 \\
& Overall, this lense is awesome! & 0.93 \\
& Let me just say that this lens is simply amazing! & 0.93 \\
& All in all this is a great lens. & 0.93 \\
& The overall clarity of the lens is stunning. & 0.91 \\
& The build quality on this lens is amazing. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0375703764.jpg}}
& \textbf{but still a great book and a wonderful story.} & 1.5\\
\cmidrule{2-3}
& It's an amazing book (or maybe an a-mazing book). & 0.91 \\
& A truly memorable and exciting reading experience. & 0.89 \\
& Overall, a good read, well worth the effort. & 0.89 \\
& Great book, original, inspired and thought provoking!! & 0.89 \\
& A worthwhile read, beautiful and engaging. & 0.88 \\
& The presentation of the book is also incredible! & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0001WE6U2.jpg}}
& \textbf{Works as advertised so I'm pleased.} & 1.48\\
\cmidrule{2-3}
& Good Product, works as intended & 0.92 \\
& It was the item that I wanted and very happy with it. & 0.92 \\
& Exactly what I wanted, and it works well. & 0.92 \\
& Very happy with this purchase. & 0.91 \\
& Works great; does want it supposed to. & 0.89 \\
& This one fits perfectly and it a reasonable price. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B001SEQPGK.jpg}}
& \textbf{Has very good pic quality and extremely easy to use.} & 1.68\\
\cmidrule{2-3}
& But the ease of use and picture quality are very very easy. & 0.94 \\
& Its feature packed and easy to use. & 0.92 \\
& It is extremely easy to use and takes phenomenal pictures! & 0.92 \\
& The steady image feature is excellent and gives really crispy images. & 0.92 \\
& This is a good product with easy use and intelligent features which makes it use at any location and anytime. & 0.89 \\
& The camera is nicely built with easy to use controls. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00XI057M0.jpg}}
& \textbf{This is one of the best Sci-Fi films of the year, of recent memory and of thelast decade, as well, too.} & 1.57\\
\cmidrule{2-3}
& I thought this was one of the best sci-fi movies in years. & 0.93 \\
& One of the best sci-fi movies I've seen in a while. & 0.9 \\
& One of the best Sci-Fi movies I've ever seen. & 0.9 \\
& OVERALL: EX MACHINA is one of the best films this year so far. & 0.89 \\
& [Originally posted at JustPressPlay.net]king for a solid and above par Sci-Fi film to support, Ex Machina is the best we’ve seen all year. & 0.88 \\
& If you were looking for a solid and above par Sci-Fi film to support, Ex Machina is the best we’ve seen all year. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00005LEOH.jpg}}
& \textbf{This lens is great, and iffy at the same time.} & 1.62\\
\cmidrule{2-3}
& Goddamn this is a wonderful lens. & 0.93 \\
& Make no mistake, it's a great lens. & 0.92 \\
& Thanks you very much, what a great lens! & 0.91 \\
& The pictures are just stunning . & 0.89 \\
& It's very well constructed and takes great picture too. & 0.89 \\
& Reflection control is wonderful. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0061ZFWBU.jpg}}
& \textbf{They are a great color, they have great sound quality and they are comfortable!} & 1.7\\
\cmidrule{2-3}
& These fit their heads comfortably and the colors are terrific. & 0.94 \\
& The sound quality is very good. & 0.92 \\
& They work great and the sound is pretty good! & 0.92 \\
& They sound great and they are very comfortable. & 0.92 \\
& Good connection and decent sound quality. & 0.91 \\
& I also tried them and they are very comfortable and the sound is great. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B003IHUHGE.jpg}}
& \textbf{Very high quality sound and comfortable on the ears.} & 1.69\\
\cmidrule{2-3}
& The fit is super comfortable and the sound is unbelievable. & 0.93 \\
& They are very comfortable, the sound is excellent. & 0.93 \\
& excellent balanced sound, very comfortable. & 0.92 \\
& Very natural, high quality sound. & 0.92 \\
& They provide such beautiful and rich sound. & 0.9 \\
& The headset looks just as great as it sounds and is extremely comfortable. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00000J0JF.jpg}}
& \textbf{It's a good think-ahead game and we all have fun playing it.} & 1.57\\
\cmidrule{2-3}
& I really enjoy playing this game. & 0.94 \\
& This is a great concept and fun to play. & 0.93 \\
& It is these moments that make the game so much fun to play. & 0.93 \\
& The game is well constructed, holds his interest and in his words I really like to play it. & 0.92 \\
& We all enjoy playing this together. & 0.92 \\
& The game is lots of fun and makes you think strategically. & 0.92 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00005QT9O.jpg}}
& \textbf{This is one of my favorite movies, and no Christmas is complete without this.} & 1.48\\
\cmidrule{2-3}
& Le P\&egrave;re Noël Est Une Ordure is one of my favorite movies OF ALL TIME, and my very favorite Christmas movie! & 0.93 \\
& This is my favorite Christmas movie! & 0.93 \\
& This is my favorite Holiday movie. & 0.91 \\
& Our favorite Christmas movie ever! & 0.9 \\
& This is our favorite holiday movie! & 0.9 \\
& One of my favorite Christmas movies... & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/1402241372.jpg}}
& \textbf{This is an excellent story - a very engaging read.} & 1.56\\
\cmidrule{2-3}
& Well written and a great read. & 0.95 \\
& This was fantastically refreshing read! & 0.94 \\
& All in all, a very satisfying book! & 0.93 \\
& A very engaging story and great characters & 0.91 \\
& I enjoyed this book very much! & 0.91 \\
& I thoroughly enjoyed this book. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B001196MG0.jpg}}
& \textbf{Looks very good and is packaged very well.} & 1.5\\
\cmidrule{2-3}
& And it ships well, and holds up well under use. & 0.94 \\
& The actual product is quite good. & 0.92 \\
& Arrived in great time and was very well packaged. & 0.91 \\
& Excellent quality and versatility. & 0.9 \\
& I like it because it is of great quality, and it is consistent. & 0.9 \\
& Over all This seems to make a good screen. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B007R3AZNK.jpg}}
& \textbf{I loved the music and his performance was amazing.} & 1.49\\
\cmidrule{2-3}
& The guy is a great musician and really shows that on this CD. & 0.91 \\
& My husband and I love the music this man plays. & 0.91 \\
& The talent of these musicians is so great. & 0.89 \\
& It is such a joy to listen to him play! & 0.89 \\
& great songs and great musicians! & 0.89 \\
& Joe does a great job bringing the tunes to life and filling them with feeling and soul. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0451414047.jpg}}
& \textbf{I truly enjoyed the book-it is a great tribute to Selena and I feel her fans will love it.} & 1.52\\
\cmidrule{2-3}
& I truly enjoyed reading this book and I recommend it to anyone who's a Selena fan. & 0.94 \\
& Thank you Chris for writing this and sharing to her fans just how much she of a truly amazing person she was and forever will be. & 0.91 \\
& This book was so great I love selena and I will read this book over and over again because i get to hear more about selena & 0.9 \\
& Anyone who loves Selena (and yes, I use present tense) will love this book...thank you so much, Chris. & 0.9 \\
& Anyone who is a true fan of Selena's will treasure this because as you're reading, it's like she's alive again. & 0.9 \\
& It's really a great book and I feel so much closer to Chris and Selena after reading this. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000ANVPP6.jpg}}
& \textbf{This is one of John Wayne's best movies !!!!} & 1.51\\
\cmidrule{2-3}
& Excellent movie - perhaps one of the best Wayne has acted in, in my opinion. & 0.93 \\
& this is a really good john wayne movie. & 0.91 \\
& This is the best movie John Wayne ever made. & 0.9 \\
& one of his better movies.. would day this is very good movie for any John Wayne fan.. & 0.9 \\
& This is one of John Wayne's better movies. & 0.87 \\
& John Wayne is one of my favorite actors. & 0.86 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00092KD9C.jpg}}
& \textbf{This is a very comfortable strap and is constructed very well.} & 1.62\\
\cmidrule{2-3}
& The strap is very comfortable to wear. & 0.95 \\
& Most importantly it is very comfortable. & 0.95 \\
& They both are extremely comfortable and secure. & 0.94 \\
& This strap is well made, super comfortable, and appears to be very strong. & 0.94 \\
& Very comfortable and is highly recommended! & 0.92 \\
& Either way, this strap is well made and does the job. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0790731886.jpg}}
& \textbf{this has to be one of my favorite movies ever made , way too funny.} & 1.5\\
\cmidrule{2-3}
& This is one of my all time favorite movie really fun. & 0.92 \\
& One of my favorite all time movies! & 0.89 \\
& We loved Arthur when it first came into the movies, and  it is still one of the funniest movies there is. & 0.88 \\
& a great classic comedy movie and i like it alot & 0.87 \\
& This movie is still one of the funniest movies ever and with the most memorable, repeatable lines. & 0.87 \\
& My all-time favorite comedy movie. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B008MPKAPK.jpg}}
& \textbf{Excellent small radio with great sound.} & 1.67\\
\cmidrule{2-3}
& Great sound for a small radio. & 0.97 \\
& It has a really good sound for a small radio. & 0.96 \\
& Great reception for such a small radio. & 0.95 \\
& Hello this is a very nice small radio but has great sound to it. & 0.92 \\
& This radio is small and works well. & 0.92 \\
& This is what it claims, a small radio that works pretty well. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B003RHZ66Q.jpg}}
& \textbf{A Fashion Fairy Tale is another delightful, entertaining Barbie movie that I highly recommend for the whole family.} & 1.55\\
\cmidrule{2-3}
& I have a daycare home and all of the children love Barbie, this is a very good movie. & 0.9 \\
& Ok, I like all the Barbie Movies, but this one is special, absolutely my favorite! & 0.89 \\
& Barbie: A fashion fairytale is a fun movie with awesome animation, music and a great voice cast! & 0.88 \\
& My daughter LOVES Barbie movies, so of course this one was on her Christmas list! & 0.88 \\
& She loved the idea that fashion design is actually a career, and the DVD extras included an interview with a real fashion designer that works on Barbie. & 0.88 \\
& we love Barbie especially the ones that have Kelly Sheridan! & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B001NESPHC.jpg}}
& \textbf{Melody Gardot has a great voice and I love many of the songs.} & 1.48\\
\cmidrule{2-3}
& Melody has very good melodies for these songs and she sings them beautifully. & 0.94 \\
& Her song-writing abilities are fantastic and bring a lot of depth to the songs. & 0.92 \\
& Her voice is incredible, the lyrics are fantastic. & 0.92 \\
& One of the great things about Gardot is also the fact that she can and does SING her songs. & 0.91 \\
& I am a fan of the standards, and her voice is fabulous. & 0.89 \\
& Melody's voice and lyrics are stunning. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000OG88NQ.jpg}}
& \textbf{They have good sound quality and were very easy to set up.} & 1.66\\
\cmidrule{2-3}
& On a positive note returning the speakers was easy. & 0.92 \\
& The sound is clean and the center works very well. & 0.91 \\
& This inexpensive unit did the job perfectly. & 0.89 \\
& Decent sound, stylish design, small size made this an easy choice. & 0.88 \\
& These little speakers are perfect, very cute and produce clear sound and we couldn't be happier with our purchases. & 0.87 \\
& It works and the sound quality is good. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00NAPJ8DM.jpg}}
& \textbf{They work great with the Lego's we already have.} & 1.51\\
\cmidrule{2-3}
& They are great quality and work with Lego brand! & 0.92 \\
& It works just like of the Legos. & 0.92 \\
& The ones that do fit together work fine with all Legos and are just like legos. & 0.92 \\
& And they do work fine with Lego brand, so it's a great way to expand your collection. & 0.92 \\
& Almost as good as Lego's and seems to be quite compatible with them. & 0.91 \\
& Pieces were high quality and Fit fine with Lego. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0761165975.jpg}}
& \textbf{It is a great tool for helping to plan your wedding.} & 1.58\\
\cmidrule{2-3}
& Was a great help in planning my wedding! & 0.94 \\
& This came in SO handy for planning my wedding! & 0.93 \\
& It helps you decide what type of wedding and provides great suggestions. & 0.92 \\
& But all in all, I think this was a great way to get a feel for planning a wedding. & 0.92 \\
& The planner / organizer is very thorough and will be helpful to see from the bride's perspective about planning a wedding. & 0.91 \\
& Very useful tool for wedding planners & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0062065254.jpg}}
& \textbf{As I got in to the book, I found the people interesting, the characters believable and genuinely liked the book.} & 1.45\\
\cmidrule{2-3}
& I liked the descriptions and thought the novel was very believable. & 0.92 \\
& Our book club really enjoyed the discussion. & 0.9 \\
& My book club picked this book and really enjoyed it. & 0.9 \\
& Love this book, love this author, she can really engage the reader and bring us into a world most of us are not privy to. & 0.88 \\
& The writer's style was easy to read and kept me interested. & 0.87 \\
& This was a local bookclub selection and I really enjoyed the story. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B004BFVKSQ.jpg}}
& \textbf{my girl like it and i like it sooooo much, the quality is excellent, very nice doll i want to buy more of it} & 1.62\\
\cmidrule{2-3}
& She is a beautiful doll that will bring a lot of joy to the girl who receives this. & 0.91 \\
& Great size, cute box, love the accessories my little niece will be so happy!! & 0.9 \\
& The doll is very cute and seems to be fun for my granddaughter. & 0.88 \\
& My daughter loves this Punzel doll! & 0.87 \\
& My granddaughter loves this doll. & 0.87 \\
& This doll was nicely packaged and an immediate favorite! & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000L212HC.jpg}}
& \textbf{This is a fantastic movie with great acting.} & 1.57\\
\cmidrule{2-3}
& What a great movie, what an awesome cast! & 0.96 \\
& This is a great movie with terrific acting and a compelling plot. & 0.95 \\
& A wonderful and well acted movie. & 0.94 \\
& Great story line and fantastic acting. & 0.92 \\
& It's a good movie with a lot of stars, a very good script and an rare end. & 0.92 \\
& The film was well done,  very creative and well acted. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000002KHF.jpg}}
& \textbf{I love Van Morrison and this CD along with Astral Weeks is his best work by far.} & 1.51\\
\cmidrule{2-3}
& This is a must have CD, if only for \&quot;caravan\&quot; Morrison's best song ever. & 0.89 \\
& Van Morrison is an incredible artist, and this truly is my favorite set of works by him. & 0.89 \\
& All of Van Morrison's songs are great...but this album will always be my favorite. & 0.89 \\
& If you love classic van then you will love this album  it portrays van at his best. & 0.88 \\
& What can I say, the song Moondance is so romantic <;3 I think this is Van Morrison's best album, it's a classic. & 0.88 \\
& this is one of Morrison's best albums...he lets everyone join in \&quot;the mystic.\&quot;  Really keeps the momentum going from the timeless \&quot;Astral Weeks.\&quot; & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00B0DWB62.jpg}}
& \textbf{Overall it is very cute and the kids had a great time with it.} & 1.46\\
\cmidrule{2-3}
& Very durable and the kids love it! & 0.92 \\
& All in all, we are quite happy with it as a toy. & 0.92 \\
& Little one LOVES it, so much to do!! & 0.89 \\
& Easy to put together \& very happy with the quality. & 0.89 \\
& Grand kids love playing with it. & 0.89 \\
& It is very colorful and really cute. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000ONDRFS.jpg}}
& \textbf{this is such a great product and very easy to use.} & 1.62\\
\cmidrule{2-3}
& This is SO easy to use and does a great job. & 0.99 \\
& It is so easy to use and handy! & 0.97 \\
& This is the best and so easy to use. & 0.96 \\
& It is surprisingly easy to use. & 0.94 \\
& The picture is very clear and it's easy to use. & 0.94 \\
& It's so convenient and accessible. & 0.93 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0002MQGR2.jpg}}
& \textbf{Installed easily, and works perfectly in this application.} & 1.62\\
\cmidrule{2-3}
& This device works perfectly for my application! & 0.92 \\
& It's working perfectly and doing exactly what I needed. & 0.9 \\
& The splitter works exactly as I expected. & 0.88 \\
& This product does on work at all. & 0.87 \\
& This thing works perfectly IF you're using the correct setup. & 0.86 \\
& This works very well for that purpose and we have had no problems with it. & 0.86 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0553386697.jpg}}
& \textbf{the material is so easy to apply...great stuff and a must read.} & 1.58\\
\cmidrule{2-3}
& Easy to read and very informative. & 0.91 \\
& This is very easy to read and understand. & 0.91 \\
& Very readable, well written and interesting. & 0.9 \\
& A true gift thats an easy read. & 0.9 \\
& Like the way it is written, easy to understand. & 0.9 \\
& Nice easy read and good information. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00023GGHQ.jpg}}
& \textbf{i treasure this cd and loved the movie!!} & 1.5\\
\cmidrule{2-3}
& I love this movie and soundtrack. & 0.94 \\
& I like the movie and I love the CD. & 0.94 \\
& I love the CD almost a much as I loved the movie. & 0.93 \\
& With that being said, personally I love the soundtrack and the movie. & 0.92 \\
& I enjoyed the film ... but I LOVED the soundtrack. & 0.9 \\
& I loved the music on this soundtrack so much! & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000UJBY4W.jpg}}
& \textbf{This is a very good collection of some of the best songs from one of the best bands of all time - Chicago.} & 1.53\\
\cmidrule{2-3}
& All the very best of this amazing band, this classic Chicago material appeals to the very connoisseur of that Musical era. & 0.91 \\
& To any Chicago fans looking for some fantastic music, Chicago II and Chicago Transit Authority (respectively) provide the best listening experience with any album I've ever listened to. & 0.89 \\
& Rhino and Chicago have done their very best to showcase one of the Windy City's most successful bands. & 0.89 \\
& I own all Chicago Music, this is one of the best mixes I have heard. & 0.88 \\
& The best of Chicago 40th aniversary is a very good compilation of Chicago's hits. & 0.88 \\
& If you are new to Chicago (the band) this album is an excellent source of hit music it even includes some music from XXX album. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0061235970.jpg}}
& \textbf{My Granddaughter loves the Fancy Nancy books and they are all a hit.} & 1.37\\
\cmidrule{2-3}
& My granddaughter loves Fancy Nancy and this book is a fun, sweet story about two good friends. & 0.92 \\
& She loves it and so do I.  She has several Fancy Nancy books and each is enterting and delightful! & 0.92 \\
& Cute book, our daughter loves Fancy Nancy, great children's book!! & 0.92 \\
& My daughter loves the Fancy Nancy collection of books. & 0.92 \\
& Don't get me wrong, it's a great story, and she loves Fancy Nancy books. & 0.91 \\
& I love these fancy Nancy books and think they are adorable and sweet. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

% \begin{tabular}{@{}lp{120mm}r@{}}
% \multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000ANVPPQ.jpg}}
% & \textbf{Well filmed, top quality acting, and wonderful sequences make this an all around great movie... an absolute classic... and one of my favorite John Wayne movies.} & 1.61\\
% \cmidrule{2-3}
% & Favorite John Wayne movie, really great one. & 0.92 \\
% & I love John Wayne movies and this is one of my favorites. & 0.9 \\
% & One of the best John Wayne movies ever made!!! & 0.89 \\
% & It is one of my ALL time favorite John Wayne films. & 0.89 \\
% & I consider this to be one of John Wayne's finest movies. & 0.88 \\
% & This is one of the best John Wayne movies that I have ever seen. & 0.88 \\
% \midrule
% \end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0011000R6.jpg}}
& \textbf{It is a very nice flash diffuser for the pop-up flash.} & 1.63\\
\cmidrule{2-3}
& excellent pop-up flash diffuser. & 0.92 \\
& The light quality is very good as fill flash. & 0.91 \\
& Pros:  Diffuses the light from my flash very well. & 0.9 \\
& Usefulness: Makes the built in pop-up flash actually useful! & 0.89 \\
& I am very impressed with how this helps the built-in flash match the character of the off camera flash. & 0.89 \\
& As for the product itself, it does a great job of softening the light front he on-board flash. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000IHY9UM.jpg}}
& \textbf{A great workout and its a lot of fun.} & 1.52\\
\cmidrule{2-3}
& It is fun and a great workout! & 0.98 \\
& It appears to be a great workout. & 0.93 \\
& overall, the workout was fun and up beat. & 0.92 \\
& Doing well...love the workout... & 0.9 \\
& They are very good exercise as well. & 0.9 \\
& This is a great workout for anyone. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B004UKNJCM.jpg}}
& \textbf{Overall it is a fun game and young kids will like it.} & 1.55\\
\cmidrule{2-3}
& Overall, it is a great game that can grow with your kids. & 0.91 \\
& Once you learn how to play it, this game is quite fun! & 0.9 \\
& The sounds are fun, and the gameplay offers great variety of clever actions and outcomes. & 0.89 \\
& so this game keeps us both happy. & 0.88 \\
& This game was entertaining and similar to the game clue. & 0.88 \\
& The kids loved this game at the beginning and still play it here and there, so that it was a good purchase. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00IUAAJY4.jpg}}
& \textbf{Anyways, looks like a great product and the directions are easy to follow.} & 1.56\\
\cmidrule{2-3}
& The instructions were easy to follow. & 0.93 \\
& That said, the directions are clear, the samples and suggestions are very helpful as well. & 0.92 \\
& Very easy to use and customer service was great when I had a question about the process. & 0.88 \\
& The quality of the final product is very good, and when we requested a page correction, customer service was excellent and responsive. & 0.87 \\
& This product is easy to use right out of the box. & 0.87 \\
& This was easy for the grand kids to do. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0015450T6.jpg}}
& \textbf{The assembly was easy, the instructions were very clear, and the proper positioning is easy to achieve.} & 1.64\\
\cmidrule{2-3}
& Good product, easy to setup, easy to work with. & 0.95 \\
& I was not disappointed, it was packaged well, and instructions were clear and easy to follow. & 0.95 \\
& The images are wonderful and the kit is very easy to set up. & 0.94 \\
& It is very easy to put together and work with. & 0.94 \\
& Instructions were easy to follow for assembly. & 0.94 \\
& The kit comes packed very nicely and setup is easy. & 0.93 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00004RD54.jpg}}
& \textbf{This is probably the best live rock album ever.} & 1.51\\
\cmidrule{2-3}
& One of the best live rock albums of my time. & 0.93 \\
& This is the best live album and one of Reed's best albums ever. & 0.92 \\
& Especially  with the two extra songs, Rock and Roll Animal is one of the greatest live  albums of all time. & 0.91 \\
& Lou Reed-Rock N Roll Animal ****  When first off this is one of the best and clearest sounding live albums of all time. & 0.9 \\
& Definitely one of the all time greatest rock albums, not just live albums. & 0.89 \\
& My favorite live rock track of all time. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B002NKM4C2.jpg}}
& \textbf{It feels well made and sounds terrific.} & 1.59\\
\cmidrule{2-3}
& Sounds great and nice features. & 0.95 \\
& I am very happy with the set up. & 0.93 \\
& Sounds good, I am enjoying it very much. & 0.92 \\
& I am very pleased and would definitely recommend. & 0.91 \\
& Great  product and excellent service, thank you! & 0.9 \\
& Excellent service, excellent equipment. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B008CQVSXC.jpg}}
& \textbf{They fit great, sound great, and look great.} & 1.64\\
\cmidrule{2-3}
& It was great, came in good condition. & 0.92 \\
& The package is so well designed and nicely done. & 0.91 \\
& Comes in very handy in every way. & 0.88 \\
& The sound is really, really great, I would recommend this product.. & 0.88 \\
& Real clear sound, really enjoy them. & 0.88 \\
& The sounds quality is very good as to be expected by Beats! & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00CKH9URU.jpg}}
& \textbf{My son really enjoys this toy, it plays with it a lot and it seems well made.} & 1.54\\
\cmidrule{2-3}
& My son loves this thing were getting lots of play out of it It's a two part toy talks makes sounds all and all a great toy & 0.94 \\
& Excellent, my son loves this toy & 0.93 \\
& The light up effect and sound effects are pretty neat and respond to motion, which my son seems to enjoy a lot. & 0.9 \\
& My son loved it .it's good  size for him . & 0.88 \\
& It's very safe to play with and my grandson has been enjoying it. & 0.88 \\
& Good size and my son loves the sound effects & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0093IZSGG.jpg}}
& \textbf{The sound is very good, particularly for such a small speaker.} & 1.63\\
\cmidrule{2-3}
& Sound quality is good for such a small speaker. & 0.96 \\
& Sound is pretty good for how small the speaker is. & 0.92 \\
& But for a small speaker it sounds great. & 0.92 \\
& Wow....great sound for a small inexpensive device. & 0.91 \\
& Decent sound for a little speaker. & 0.9 \\
& Great sound from such a lightweight small speaker. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0399162089.jpg}}
& \textbf{This coloring book is Awesome!} & 1.55\\
\cmidrule{2-3}
& This is a great coloring book. & 0.95 \\
& I am very enthusiastic about this coloring book. & 0.94 \\
& I absolutely love this coloring book. & 0.91 \\
& Unique and refreshing coloring book. & 0.89 \\
& I LOVE this creative coloring book and its amazing art! & 0.88 \\
& This coloring book satisfies my needs! & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0783225482.jpg}}
& \textbf{great movie, very funny and well acted} & 1.61\\
\cmidrule{2-3}
& This is a great movie \& very funny. & 0.97 \\
& This movie is funny and very entertaining. & 0.96 \\
& Great, funny movie with great stars. & 0.95 \\
& Anyway, back to the movie: it is so funny and the stars are so good! & 0.93 \\
& This is one of a kind movie with great star cast and they all are very very funny. & 0.91 \\
& This is a great movie for lots of laughs. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00766BEZG.jpg}}
& \textbf{Battery fits well and seems to work well.} & 1.66\\
\cmidrule{2-3}
& The Grace battery pack works very good. & 0.94 \\
& This battery works very well for its intended purpose. & 0.93 \\
& Good battery, works well with correct voltage and amp ratings. & 0.92 \\
& It fit in the battery compartment nicely and is working fine. & 0.91 \\
& the battery is perfect....it was very easy to install & 0.9 \\
& It was easy to install and so far it's working good. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0553391135.jpg}}
& \textbf{As always Debbie Macomber has written a sweet book that entertains and makes you glad you've taken the time to read it.} & 1.51\\
\cmidrule{2-3}
& Thank you Debbie Macomber for a well-written series of books that not only can entertain us, but empowers us too. & 0.91 \\
& The book flows well and kept my attention- just a fun read that leaves you with happy thoughts once you are done. & 0.9 \\
& another great story from Mrs. Macomber...can't wait till the next one...she has the knack for keeping it flowing and interesting...delivery was great and book was in great condition... & 0.89 \\
& Debbie Macomber is such a good writer and her characters become friends. & 0.89 \\
& If you are a fan of Debbie Macomber you will enjoy this book! & 0.88 \\
& I love Debbie Macomber and I love her books. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0671700758.jpg}}
& \textbf{It's an excellent book that I highly recommend.} & 1.54\\
\cmidrule{2-3}
& This has been a great read so far and is very inspiring. & 0.91 \\
& I love it and I highly recommend this. & 0.88 \\
& I highly recommend reading this! & 0.88 \\
& It is a truly EXCELLENT and timeless self improvement book!! & 0.88 \\
& It is a very informative book and I highly recommend it to everyone! & 0.88 \\
& It is good common sense, to the point and well written. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000BN8Y2W.jpg}}
& \textbf{The quality is great and so are the details.} & 1.61\\
\cmidrule{2-3}
& The quality is amazing...the details are outstanding. & 0.96 \\
& I am really pleased with the quality. & 0.94 \\
& The quality is absolutely amazing. & 0.93 \\
& It was very well constructed and very realistic. & 0.92 \\
& Very realistic and great quality! & 0.91 \\
& The material is of very good quality. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00007E7K9.jpg}}
& \textbf{Excellent bag, very sturdy and of very good quality.} & 1.66\\
\cmidrule{2-3}
& Overall, it is sturdy and well-built. & 0.92 \\
& FITS and is super great and sturdy. & 0.92 \\
& Material is very durable and zippers are of excellent quality. & 0.91 \\
& The quality of the bag exceeded my expectations - well crafted and sturdy. & 0.91 \\
& Very sturdy, high grade fabric. & 0.9 \\
& Overall, the bag has held up quite well. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B008FSCNTK.jpg}}
& \textbf{This is an excellent CD - production values are great, and the songs and stylings are what you would expect from Diana Krall.} & 1.6\\
\cmidrule{2-3}
& I love Diana Krall and this CD is an amazing collection of songs. & 0.91 \\
& This is a highly entertaing Cd and Diana Krall is at her very best. & 0.89 \\
& Another really good Diana Krall CD. & 0.89 \\
& Same great voice and music from Diana Krall. & 0.88 \\
& I am a big Diana Krall fan and this is a good album. & 0.88 \\
& She's wonderful and this CD is too. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000002KB8.jpg}}
& \textbf{It is actually very good and this is their best CD in my oppinion.} & 1.52\\
\cmidrule{2-3}
& This is a great CD, no doubt about it. & 0.91 \\
& Overall, this is a very strong debut and certainly one of their best albums. & 0.91 \\
& This album in my opinion has some of their best music. & 0.9 \\
& Anyway this album is an awesome debut, all the songs are great. & 0.9 \\
& This album is a true classic, and as good then as it is now. & 0.9 \\
& This is one of their best albums. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0618871713.jpg}}
& \textbf{In fact this book has wonderful depth and the illustrations are an integral part of a superb whole.} & 1.57\\
\cmidrule{2-3}
& It does so with incredible tenderness and understanding which the author's words and illustrations convey beautifully. & 0.9 \\
& It is skillfully done and the format perfectly enhances Bechdel's story. & 0.88 \\
& Wonderfully illustrated with fun, smart writing. & 0.87 \\
& The drawing throughout is very well done. & 0.87 \\
& The words and pictures are seamlessly intertwined into a well-crafted, interesting book. & 0.87 \\
& And the drawings are wonderful, as always. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0002COTDA.jpg}}
& \textbf{It is great to watch these again, and I highly recommend them.} & 1.54\\
\cmidrule{2-3}
& We thoroughly enjoy the series! & 0.91 \\
& We having really enjoyed them. & 0.9 \\
& I am really glad to have purchased these. & 0.9 \\
& I loved it and your service was great. & 0.9 \\
& Overall, an EXCELLENT compilation that I would highly recommend to anyone! & 0.88 \\
& I loved the Columbo seires and still do! & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0015DNIOG.jpg}}
& \textbf{Works great, and this seller was extremely accommodating.} & 1.57\\
\cmidrule{2-3}
& The order and delivery was excellent. & 0.91 \\
& I was very pleased with the purchase of this item. & 0.9 \\
& All in all I am happy with my purchase. & 0.89 \\
& Happy with the delivery and the product. & 0.87 \\
& Works flawlessly and worth the additional cost. & 0.87 \\
& They are well made, take great photos, and are durable, given reasonable care. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00AR1G3FS.jpg}}
& \textbf{very good video and sound quality as expected!} & 1.67\\
\cmidrule{2-3}
& Very good video and audio quality. & 0.92 \\
& Very good Audio and video quality. & 0.92 \\
& This very well done for sound and video. & 0.91 \\
& Video and sound quality outstanding. & 0.91 \\
& Video and sound are outstanding. & 0.9 \\
& This is a fine performance well executed and wonderfully filmed. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0399157867.jpg}}
& \textbf{I love Sue Grafton and enjoy all her books.} & 1.44\\
\cmidrule{2-3}
& As an avid fan and faithful reader of Sue Grafton's books, I started 'V' with delight. & 0.91 \\
& I love to read and I have read all of Sue Grafton's book. & 0.9 \\
& Still, I really enjoyed the book, as I do all Grafton's works. & 0.89 \\
& I really, really enjoy the Kinsey Millhone mysteries and always recommend Sue Grafton to those I know. & 0.89 \\
& Always enjoy reading Sue Grafton's books and look forward to each years new one. & 0.88 \\
& a great writer, keeps you involved in the story and you believe the characters, wonderful writer, love her books, great buy & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00DPKQ60A.jpg}}
& \textbf{Ariana has a great voices and almost all her songs are amazing!} & 1.54\\
\cmidrule{2-3}
& Her Voice is Incredible and the more and more i see her,She is just a Fantastic Singer! & 0.93 \\
& Live all the songs she is special girl with amazing voice just wow perfect ! & 0.93 \\
& The melodies, lyrics, and her voice is just so great! & 0.91 \\
& Ariana has a truly amazing voice - extremely talented. & 0.91 \\
& Ariana has an amazing voice and she has very strong vocals. & 0.91 \\
& She is enjoying it very much and can pretty much sing along with most of the songs. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0065WM4PQ.jpg}}
& \textbf{For the price it's definitely worth it!} & 1.48\\
\cmidrule{2-3}
& For the price though, I think it's great. & 0.92 \\
& Overall for the price it's a great deal \& has done well. & 0.91 \\
& Highly recommend, especially for the price. & 0.88 \\
& Very pleased with the purchase. & 0.88 \\
& Overall, I am happy with the purchase and the price. & 0.87 \\
& Besides that it's a great item to have. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00000JZC7.jpg}}
& \textbf{I love this CD it is absolutely excellent.} & 1.54\\
\cmidrule{2-3}
& Simply a great CD I would recommend. & 0.9 \\
& Love every song--its simply 'Beautiful!' & 0.9 \\
& I still find myself loving the CD. & 0.9 \\
& The true test of a wonderful CD. & 0.9 \\
& This cd is an incredible listening experience! & 0.88 \\
& The title track is simply gorgeous. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0042FDCMM.jpg}}
& \textbf{Finding this workout was wonderful.} & 1.33\\
\cmidrule{2-3}
& Easy on the body, and a great workout! & 0.9 \\
& I like the fact that anyone can do this workout. & 0.89 \\
& Both entertaining and a good workout. & 0.89 \\
& I love this level of fitness also. & 0.88 \\
& The stretching segments are great. & 0.87 \\
& They are all great and worth the time to do. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0000658L4.jpg}}
& \textbf{The pizza is adorable and my grandaughter loves to serve the pizza with the different toppings.} & 1.47\\
\cmidrule{2-3}
& He loves to serve you pizza, with your special toppings. & 0.96 \\
& My son loves to make pizza and I enjoy to pretending to eat them over and over and over. & 0.92 \\
& It's very durable, the topping combinations are endless and my son loves to cut it up and serve it with the pizza slicer. & 0.91 \\
& This toy was a hit my kids love creating their own party pizza. & 0.91 \\
& She loves putting the different toppings on the pizza and serving to her mom and dad. & 0.91 \\
& My kids like cooking their pizza, and we have given this as a gift. & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B003T90WY8.jpg}}
& \textbf{I find they are comfortable and work quite well.} & 1.59\\
\cmidrule{2-3}
& He says they are very comfortable and do the job well. & 0.96 \\
& These are perfect and hey are comfortable. & 0.94 \\
& They attach easily and fit comfortably. & 0.93 \\
& Actually the product fits and works very well. & 0.92 \\
& They're very flexible and comfortable. & 0.92 \\
& I'm very pleased with how well they work. & 0.92 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000AO3L84.jpg}}
& \textbf{The flash is easy to learn and use.} & 1.66\\
\cmidrule{2-3}
& This flash is easy to use and has lots of extras. & 0.93 \\
& Very easy to use and highly recomended for flash photography. & 0.91 \\
& The flash is great- smooth swivel and easy to use manual and TTL functions. & 0.91 \\
& It is easy to use and found that bouncing the flash opens up a world of possibilities. & 0.89 \\
& Very easy to use and works great. & 0.89 \\
& It's very easy to use, and works great with the Canon XSI. & 0.89 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B006KD37TC.jpg}}
& \textbf{Easy to use, good sound quality, great value proposition.} & 1.67\\
\cmidrule{2-3}
& Very easy to set up, great sound. & 0.95 \\
& easy to set up and works great & 0.93 \\
& It is well made, with quality parts, and is attractive and sounds just great. & 0.92 \\
& Easy setup outstanding reception. & 0.92 \\
& However, it was easy to set up and has performed very well. & 0.92 \\
& All in all, a very nice product, with good product support. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B000OVLBFS.jpg}}
& \textbf{I love the Jesse Stone books, and have really enjoyed all the Jesse Stone movies that Tom Selleck has made.} & 1.53\\
\cmidrule{2-3}
& I like all the Jesse Stone movies and enjoy watching them again. & 0.92 \\
& I enjoyed all the Jesse Stone movies. & 0.91 \\
& I love the Jesse Stone movies and Tom Selleck in the role. & 0.89 \\
& Liked the interaction between Tom Selleck and the other characters in all the Jesse Stone movies. & 0.88 \\
& Love the Jesse Stone movies and bought a bunch-in series-so I could watch them over and over again. & 0.88 \\
& Love all the Jesse Stone movies. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0017O3UHI.jpg}}
& \textbf{Overall, we are very pleased with this antenna and would highly recommend it!} & 1.57\\
\cmidrule{2-3}
& Overall, I am extremely satisfied with this antenna. & 0.93 \\
& But I was so happy with this antenna that I wanted to give my opinion of it. & 0.92 \\
& Overall though I'm incredibly happy with the antenna. & 0.91 \\
& I am very pleased with my product. & 0.9 \\
& I highly recommend this product! & 0.88 \\
& Overall, I like the antenna for it's improved consistent signal. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00013M6NU.jpg}}
& \textbf{so I ordered this and it worked just fine.} & 1.37\\
\cmidrule{2-3}
& I ordered this used one and it works perfectly. & 0.92 \\
& This is exactly what I had before and it works great. & 0.9 \\
& I mean it's OEM so it works fine. & 0.89 \\
& It is easy to use and does the job as advertised. & 0.88 \\
& This one works exactly as advertised. & 0.87 \\
& I am pleased with this product. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0018QROM2.jpg}}
& \textbf{This center channel speaker sounds great and looks good.} & 1.65\\
\cmidrule{2-3}
& This center channel speaker is awesome. & 0.95 \\
& Very nice center channel speaker. & 0.94 \\
& Very nice center speaker, nicely built \& great sound quality. & 0.94 \\
& It looks good and performs great. & 0.93 \\
& This is a nice unit that sounds great. & 0.93 \\
& This Center channel is great I love it. & 0.93 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00007JZVB.jpg}}
& \textbf{it's really fun and i enjoy and the overall dance routine.} & 1.54\\
\cmidrule{2-3}
& I absolutely enjoy doing this dance. & 0.95 \\
& They give an excellent workout, full of fun and serious dancing! & 0.91 \\
& This is what really makes you want to dance \& have fun. & 0.91 \\
& The performances under the special features are good to watch and get a feel for the dance. & 0.87 \\
& The two dancers are lovely to watch. & 0.86 \\
& It's so much fun to bellydance. & 0.86 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00000F1D3.jpg}}
& \textbf{This is one of the best Cher songs ever and definately one of the best from this album!} & 1.54\\
\cmidrule{2-3}
& ALL OR NOTHING  This is considered to be one of the best Cher songs of all-time, and definately a fan favourite. & 0.95 \\
& BELIEVE IS DEFINATLY THE BEST SONG CHER HAS EVER DONE. & 0.94 \\
& One of the best CD's ever made by Cher. & 0.93 \\
& THESE ARE SIMPLY THE BEST TRACKS CHER HAS PUT OUT. & 0.91 \\
& I think it is one of Cher's best albums. & 0.91 \\
& This is one of the best CDs that Cher has put out. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/014312417X.jpg}}
& \textbf{its an awesome book and has a great message.} & 1.57\\
\cmidrule{2-3}
& Great book and really motivational. & 0.94 \\
& This book is truly inspiring !! & 0.93 \\
& Anyhow, this was a highly inspirational and motivating read. & 0.93 \\
& The book was good and delivery was great. & 0.91 \\
& It's very informative, enjoyable, and well-written. & 0.9 \\
& Thoroughly enjoying the advice that this book is providing. & 0.87 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00BPEJX12.jpg}}
& \textbf{If you enjoyed Shaun of the Dead \& Hot Fuzz, then you'll love this one.} & 1.43\\
\cmidrule{2-3}
& If you like Shaun of the Dead and Hot Fuzz - you will definitely like this one. & 0.96 \\
& I loved Shaun of the dead and to a lesser extent hot fuzz. & 0.92 \\
& If you like Shaun of the Dead and Hot Fuzz, then you must see this one too. & 0.92 \\
& If you liked Shawn of the Dead, Hot Fuzz, and even Paul, you will enjoy this one too. & 0.9 \\
& If you loved Shaun of the Dead and Hot Fuzz you'll undoubtedly love The World's End. & 0.9 \\
& If you love Shaun of the dead, or Hot fuzz this is a must have. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B0007QKMQY.jpg}}
& \textbf{We are very pleased with this camera.} & 1.54\\
\cmidrule{2-3}
& The camera does very nice work. & 0.93 \\
& It was a great camera and served our purpose well. & 0.92 \\
& Camera works great and the pictures are awesome. & 0.91 \\
& We absolutely love this camera!!!!! & 0.91 \\
& Altogether, this camera is worth it. & 0.91 \\
& Is a really great camera absolutly love it. & 0.91 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00000FCBH.jpg}}
& \textbf{2pac is definetly the best rapper ever and this is the best CD he has.} & 1.53\\
\cmidrule{2-3}
& Tupac is obviously the best ever rapper. & 0.96 \\
& Tupac is definitely one of the best rapper ever lived. & 0.95 \\
& It has the best hit songs from the best rapper ever. & 0.95 \\
& 2pac is the best rapper that ever lived. & 0.94 \\
& 2pac Is The Best Rapper Ever.  & 0.94 \\
& He was truly unique, and he and B.I.G. are still the best rappers of all time. & 0.94 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B003HC9JIW.jpg}}
& \textbf{It is simple, but is a great workout.} & 1.41\\
\cmidrule{2-3}
& The moves were easy for me to do yet gave me a good workout. & 0.89 \\
& Easy to follow plus you feel like you are getting a pretty good workout. & 0.89 \\
& Great simple workout, easy to follow and not boring. & 0.89 \\
& Easy to do but really helps joints and muscles. & 0.88 \\
& Just a good, clean, effective workout. & 0.87 \\
& I love this low impact workout. & 0.86 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/0670012335.jpg}}
& \textbf{We love the Llama Llama series and this book is just as wonderful as the rest!} & 1.56\\
\cmidrule{2-3}
& Just like all the other llama llama books, this one is wonderful. & 0.93 \\
& Such a cute book - I LOVE all of the Llama Llama books! & 0.92 \\
& I love the llama llama books!. & 0.92 \\
& He loves Llama llama, and this is an excellent addition to the series. & 0.91 \\
& We love the llama llama books. & 0.91 \\
& Great book - love  the Llama books! & 0.9 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B001K5UQX0.jpg}}
& \textbf{Very happy with this purchase.} & 1.28\\
\cmidrule{2-3}
& Overall I am very pleased with this purchase. & 0.97 \\
& I was very happy with my purchase. & 0.96 \\
& Overall, I am happy with this product. & 0.94 \\
& Genuinely impressed with this thing. & 0.9 \\
& Nevertheless, I still believe it was an awesome purchase. & 0.87 \\
& Easy to use and pictures turn out great. & 0.86 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B002JSM3KQ.jpg}}
& \textbf{it is a very enjoyable game to play .} & 1.56\\
\cmidrule{2-3}
& The game was so much fun to play. & 0.94 \\
& We have so much fun playing this game. & 0.92 \\
& It's a game that's meant to be played, and this version is very playable. & 0.92 \\
& But, dangit, it's just such a fun game! & 0.89 \\
& Great release of a great game. & 0.88 \\
& the members  have goodtime enjoying this game. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B008B68IUY.jpg}}
& \textbf{My granddaughter absolutely loved it!} & 1.42\\
\cmidrule{2-3}
& sure my granddaughter will love this. & 0.93 \\
& My niece wanted it and loves it. & 0.91 \\
& Granddaughter loved it and wants more, more, more! & 0.9 \\
& My niece will be so happy to play it! & 0.89 \\
& Great size and color my niece loved it & 0.89 \\
& This machine very glad, my daughter, she high glad and constantly plays with them. & 0.88 \\
\midrule
\end{tabular}

\vspace{10mm}

\begin{tabular}{@{}lp{120mm}r@{}}
\multirow{7}{32mm}{\centering\includegraphics[width=26mm,keepaspectratio]{img/B00C30FCUI.jpg}}
& \textbf{Great ear buds, great sound and comfortable.} & 1.68\\
\cmidrule{2-3}
& Good sound quality, fits comfortable in my ear & 0.94 \\
& These headphones sound superb and look damn good. & 0.92 \\
& These headphones are excellent. & 0.92 \\
& Comfortable and great sound quality. & 0.92 \\
& very good headphones overall good sound quality. & 0.92 \\
& Excellent sound, good construction on the ear bud itself. & 0.92 \\
\midrule
\end{tabular}

\vspace{10mm}


